Weird Machines as Insecure Compilation

Weird machines---the computational models accessible by exploiting security vulnerabilities---arise from the difference between the model a programmer has in her head of how her program should run and the implementation that actually executes. Previous attempts to reason about or identify weird machines have viewed these models through the lens of formal computational structures such as state machines and Turing machines. But because programmers rarely think about programs in this way, it is difficult to effectively apply insights about weird machines to improve security. We present a new view of weird machines based on techniques from programming languages theory and secure compilation. Instead of an underspecified model drawn from a programmers' head, we start with a program written in a high-level source language that enforces security properties by design. Instead of state machines to describe computation, we use the well-defined semantics of this source language and a target language, into which the source program will be compiled. Weird machines are the sets of behaviors that can be achieved by a compiled source program in the target language that cannot be achieved in the source language directly. That is, exploits are witnesses to insecure compilation. This paper develops a framework for characterizing weird machines as insecure compilation, and illustrates the framework with examples of common exploits. We study the classes of security properties that exploits violate, the compositionality of exploits in a compiler stack, and the weird machines and mitigations that arise.

==> Dullien.tex <==
% generated by Ott 0.28 from: ott/Utils.ott ott/Dullien.ott
\newcommand{\DULdrule}[4][]{{\displaystyle\frac{\begin{array}{l}#2\end{array}}{#3}\quad\DULdrulename{#4}}}
\newcommand{\DULusedrule}[1]{\[#1\]}
\newcommand{\DULpremise}[1]{ #1 \\}
\newenvironment{DULdefnblock}[3][]{ \framebox{\mbox{#2}} \quad #3 \\[0pt]}{}
\newenvironment{DULfundefnblock}[3][]{ \framebox{\mbox{#2}} \quad #3 \\[0pt]\begin{displaymath}\begin{array}{l}}{\end{array}\end{displaymath}}
\newcommand{\DULfunclause}[2]{ #1 \equiv #2 \\}
\newcommand{\DULnt}[1]{\mathit{#1}}
\newcommand{\DULmv}[1]{\mathit{#1}}
\newcommand{\DULkw}[1]{\mathbf{#1}}
\newcommand{\DULsym}[1]{#1}
\newcommand{\DULcom}[1]{\text{#1}}
\newcommand{\DULdrulename}[1]{\textsc{#1}}
\newcommand{\DULcomplu}[5]{\overline{#1}^{\,#2\in #3 #4 #5}}
\newcommand{\DULcompu}[3]{\overline{#1}^{\,#2<#3}}
\newcommand{\DULcomp}[2]{\overline{#1}^{\,#2}}
\newcommand{\DULgrammartabular}[1]{\begin{supertabular}{llcllllll}#1\end{supertabular}}
\newcommand{\DULmetavartabular}[1]{\begin{supertabular}{ll}#1\end{supertabular}}
\newcommand{\DULrulehead}[3]{$#1$ & & $#2$ & & & \multicolumn{2}{l}{#3}}
\newcommand{\DULprodline}[6]{& & $#1$ & $#2$ & $#3 #4$ & $#5$ & $#6$}
\newcommand{\DULfirstprodline}[6]{\DULprodline{#1}{#2}{#3}{#4}{#5}{#6}}
\newcommand{\DULlongprodline}[2]{& & $#1$ & \multicolumn{4}{l}{$#2$}}
\newcommand{\DULfirstlongprodline}[2]{\DULlongprodline{#1}{#2}}
\newcommand{\DULbindspecprodline}[6]{\DULprodline{#1}{#2}{#3}{#4}{#5}{#6}}
\newcommand{\DULprodnewline}{\\}
\newcommand{\DULinterrule}{\\[5.0mm]}
\newcommand{\DULafterlastrule}{\\}
\newcommand{\DULmetavars}{
\DULmetavartabular{
 $ \DULmv{index} ,\, \DULmv{i} ,\, \DULmv{j} ,\, \DULmv{n} ,\, \DULmv{m} $ &  \\
 $ x ,\, \DULmv{x} ,\, \DULmv{y} $ &  \\
}}

\newcommand{\DULdigit}{
\DULrulehead{\DULnt{digit}}{::=}{}\DULprodnewline
\DULfirstprodline{|}{\DULsym{0}}{}{}{}{}\DULprodnewline
\DULprodline{|}{\DULsym{1}}{}{}{}{}\DULprodnewline
\DULprodline{|}{\DULsym{2}}{}{}{}{}\DULprodnewline
\DULprodline{|}{\DULsym{3}}{}{}{}{}\DULprodnewline
\DULprodline{|}{\DULsym{4}}{}{}{}{}\DULprodnewline
\DULprodline{|}{\DULsym{5}}{}{}{}{}\DULprodnewline
\DULprodline{|}{\DULsym{6}}{}{}{}{}\DULprodnewline
\DULprodline{|}{\DULsym{7}}{}{}{}{}\DULprodnewline
\DULprodline{|}{\DULsym{8}}{}{}{}{}\DULprodnewline
\DULprodline{|}{\DULsym{9}}{}{}{}{}}

\newcommand{\DULnat}{
\DULrulehead{n}{::=}{}\DULprodnewline
\DULfirstprodline{|}{\DULnt{digit_{{\mathrm{1}}}} \, .. \, \DULnt{digit_{\DULmv{n}}}}{}{}{}{}}

\newcommand{\DULint}{
\DULrulehead{i}{::=}{}\DULprodnewline
\DULfirstprodline{|}{n}{}{}{}{}\DULprodnewline
\DULprodline{|}{\DULsym{-}  n}{}{}{}{}}

\newcommand{\DULbool}{
\DULrulehead{b}{::=}{\DULcom{booleans}}\DULprodnewline
\DULfirstprodline{|}{\true}{}{}{}{}\DULprodnewline
\DULprodline{|}{\false}{}{}{}{}}

\newcommand{\DULchar}{
\DULrulehead{c}{::=}{}\DULprodnewline
\DULfirstprodline{|}{ a }{}{}{}{}\DULprodnewline
\DULprodline{|}{ b }{}{}{}{}\DULprodnewline
\DULprodline{|}{ c }{}{}{}{}\DULprodnewline
\DULprodline{|}{ d }{}{}{}{}\DULprodnewline
\DULprodline{|}{ e }{}{}{}{}\DULprodnewline
\DULprodline{|}{ f }{}{}{}{}\DULprodnewline
\DULprodline{|}{ g }{}{}{}{}\DULprodnewline
\DULprodline{|}{ h }{}{}{}{}\DULprodnewline
\DULprodline{|}{ i }{}{}{}{}\DULprodnewline
\DULprodline{|}{ j }{}{}{}{}\DULprodnewline
\DULprodline{|}{ k }{}{}{}{}\DULprodnewline
\DULprodline{|}{ l }{}{}{}{}\DULprodnewline
\DULprodline{|}{ m }{}{}{}{}\DULprodnewline
\DULprodline{|}{ n }{}{}{}{}\DULprodnewline
\DULprodline{|}{ o }{}{}{}{}\DULprodnewline
\DULprodline{|}{ p }{}{}{}{}\DULprodnewline
\DULprodline{|}{ q }{}{}{}{}\DULprodnewline
\DULprodline{|}{ r }{}{}{}{}\DULprodnewline
\DULprodline{|}{ s }{}{}{}{}\DULprodnewline
\DULprodline{|}{ t }{}{}{}{}\DULprodnewline
\DULprodline{|}{ u }{}{}{}{}\DULprodnewline
\DULprodline{|}{ v }{}{}{}{}\DULprodnewline
\DULprodline{|}{ w }{}{}{}{}\DULprodnewline
\DULprodline{|}{ x }{}{}{}{}\DULprodnewline
\DULprodline{|}{ y }{}{}{}{}\DULprodnewline
\DULprodline{|}{ z }{}{}{}{}}

\newcommand{\DULform}{
\DULrulehead{\DULnt{form}}{::=}{}\DULprodnewline
\DULfirstprodline{|}{\forall  \DULnt{top_{{\mathrm{1}}}} \, .. \, \DULnt{top_{\DULmv{n}}}  .\xspace  \DULnt{form}}{}{}{}{}\DULprodnewline
\DULprodline{|}{\forall  \DULnt{judg_{{\mathrm{1}}}} \, .. \, \DULnt{judg_{\DULmv{n}}}  .\xspace  \DULnt{form}}{}{}{}{}\DULprodnewline
\DULprodline{|}{\exists\xspace  \DULnt{top_{{\mathrm{1}}}} \, .. \, \DULnt{top_{\DULmv{n}}}  .\xspace  \DULnt{form}}{}{}{}{}\DULprodnewline
\DULprodline{|}{\exists\xspace  \DULnt{judg_{{\mathrm{1}}}} \, .. \, \DULnt{judg_{\DULmv{n}}}  .\xspace  \DULnt{form}}{}{}{}{}\DULprodnewline
\DULprodline{|}{\DULnt{top}  \triangleq  \DULnt{top_{{\mathrm{2}}}}}{}{}{}{}\DULprodnewline
\DULprodline{|}{\DULnt{top}  \triangleq  \DULnt{form}}{}{}{}{}\DULprodnewline
\DULprodline{|}{\DULnt{judg}  \triangleq  \DULnt{form}}{}{}{}{}\DULprodnewline
\DULprodline{|}{\DULnt{top_{{\mathrm{1}}}}  \DULsym{=}  \DULnt{top_{{\mathrm{2}}}}}{}{}{}{}\DULprodnewline
\DULprodline{|}{\DULnt{top_{{\mathrm{1}}}}  \neq  \DULnt{top_{{\mathrm{2}}}}}{}{}{}{}\DULprodnewline
\DULprodline{|}{\DULnt{judg}}{}{}{}{}\DULprodnewline
\DULprodline{|}{\neg  \DULnt{form}}{}{}{}{}\DULprodnewline
\DULprodline{|}{\DULnt{form_{{\mathrm{1}}}}  \wedge  \DULnt{form_{{\mathrm{2}}}}}{}{}{}{}\DULprodnewline
\DULprodline{|}{\DULnt{form_{{\mathrm{1}}}}  \vee  \DULnt{form_{{\mathrm{2}}}}}{}{}{}{}\DULprodnewline
\DULprodline{|}{\DULnt{form_{{\mathrm{1}}}}  \Rightarrow  \DULnt{form_{{\mathrm{2}}}}}{}{}{}{}\DULprodnewline
\DULprodline{|}{b}{}{}{}{}}

\newcommand{\DULPXXS}{
\DULrulehead{\source{P}}{::=}{\DULcom{source whole programs}}\DULprodnewline
\DULfirstprodline{|}{s}{}{}{}{}}

\newcommand{\DULPXXT}{
\DULrulehead{\target{P}}{::=}{\DULcom{target whole programs}}\DULprodnewline
\DULfirstprodline{|}{s}{}{}{}{}}

\newcommand{\DULsstate}{
\DULrulehead{\source{q}^\source{S}}{::=}{}}

\newcommand{\DULtstate}{
\DULrulehead{\target{q}^\target{T}}{::=}{}\DULprodnewline
\DULfirstprodline{|}{ \target{q}^\target{T} _t }{}{}{}{}\DULprodnewline
\DULprodline{|}{ \target{q}^\target{T} _w }{}{}{}{}}

\newcommand{\DULstate}{
\DULrulehead{q  ,\ \DULnt{q}}{::=}{}\DULprodnewline
\DULfirstprodline{|}{\source{q}^\source{S}}{}{}{}{}\DULprodnewline
\DULprodline{|}{\target{q}^\target{T}}{}{}{}{}}

\newcommand{\DULrepmap}{
\DULrulehead{\gamma  ,\ \texttt{trans}}{::=}{}}

\newcommand{\DULQ}{
\DULrulehead{\DULnt{Q}}{::=}{\DULcom{set of states}}\DULprodnewline
\DULfirstprodline{|}{ \source{Q}_{\IFSM} }{}{}{}{}\DULprodnewline
\DULprodline{|}{ \target{Q}_{\CPU} }{}{}{}{}\DULprodnewline
\DULprodline{|}{\gamma  \DULsym{(}  \source{q}^\source{S}  \DULsym{)}}{}{}{}{\DULcom{is a subset of QIMP}}\DULprodnewline
\DULprodline{|}{ \target{Q}_{ \textsf{Sane} } }{}{}{}{}\DULprodnewline
\DULprodline{|}{ \target{Q}_{ \textsf{Trans} } }{}{}{}{}\DULprodnewline
\DULprodline{|}{ \target{Q}_{ \textsf{Weird} } }{}{}{}{}\DULprodnewline
\DULprodline{|}{Q_A}{}{}{}{}}

\newcommand{\DULAccepting}{
\DULrulehead{Q_A}{::=}{}\DULprodnewline
\DULfirstprodline{|}{ \source{Q}_{A} }{}{}{}{}\DULprodnewline
\DULprodline{|}{ \target{Q}_{A} }{}{}{}{}}

\newcommand{\DULFSM}{
\DULrulehead{\DULnt{FSM}}{::=}{}\DULprodnewline
\DULfirstprodline{|}{\DULsym{(}  \DULnt{Q}  \DULsym{,}  \Sigma  \DULsym{,}  \delta  \DULsym{,}  q  \DULsym{,}  Q_A  \DULsym{)}}{}{}{}{}\DULprodnewline
\DULprodline{|}{ \IFSM }{}{}{}{}\DULprodnewline
\DULprodline{|}{ \CPU }{}{}{}{}}

\newcommand{\DULAlphabet}{
\DULrulehead{\Sigma}{::=}{}\DULprodnewline
\DULfirstprodline{|}{ \texttt{Machine}^{ \DULnt{FSM} }( \DULnt{q} ) }{}{}{}{}\DULprodnewline
\DULprodline{|}{ \mathsource{\Sigma} }{}{}{}{}\DULprodnewline
\DULprodline{|}{ \mathtarget{\Sigma} }{}{}{}{}}

\newcommand{\DULTransition}{
\DULrulehead{\delta}{::=}{}\DULprodnewline
\DULfirstprodline{|}{ \mathsource{\delta} }{}{}{}{}\DULprodnewline
\DULprodline{|}{ \mathtarget{\delta} }{}{}{}{}}

\newcommand{\DULjudg}{
\DULrulehead{\DULnt{judg}}{::=}{}\DULprodnewline
\DULfirstprodline{|}{\DULnt{top}  \DULsym{:}  X}{}{}{}{}\DULprodnewline
\DULprodline{|}{\DULnt{top}  \in  X}{}{}{}{}\DULprodnewline
\DULprodline{|}{\DULnt{top}  \notin  X}{}{}{}{}\DULprodnewline
\DULprodline{|}{X_{{\mathrm{1}}}  \subseteq  X_{{\mathrm{2}}}}{}{}{}{}\DULprodnewline
\DULprodline{|}{ q  \oversteps{ s }  q' }{}{}{}{}}

\newcommand{\DULCmp}{
\DULrulehead{P}{::=}{\DULcom{all components}}\DULprodnewline
\DULfirstprodline{|}{\DULnt{FSM}}{}{}{}{}}

\newcommand{\DULS}{
\DULrulehead{\source{S}  ,\ \source{U}  ,\ \source{V}}{::=}{\DULcom{source components}}\DULprodnewline
\DULfirstprodline{|}{s}{}{}{}{}\DULprodnewline
\DULprodline{|}{ \IFSM }{}{}{}{}}

\newcommand{\DULT}{
\DULrulehead{\target{T}}{::=}{\DULcom{target components}}\DULprodnewline
\DULfirstprodline{|}{s}{}{}{}{}\DULprodnewline
\DULprodline{|}{ \CPU }{}{}{}{}}

\newcommand{\DULCtx}{
\DULrulehead{C}{::=}{\DULcom{program contexts}}\DULprodnewline
\DULfirstprodline{|}{q}{}{}{}{}}

\newcommand{\DULSCtx}{
\DULrulehead{\source{C}^\source{S}}{::=}{\DULcom{source program contexts}}\DULprodnewline
\DULfirstprodline{|}{\DULsym{(}  s_{{\mathrm{1}}}  \DULsym{,}  s_{{\mathrm{2}}}  \DULsym{)}}{}{}{}{}\DULprodnewline
\DULprodline{|}{\source{q}^\source{S}}{}{}{}{}}

\newcommand{\DULTCtx}{
\DULrulehead{\target{C}^\target{T}  ,\ \source{C}^\source{T}}{::=}{\DULcom{target program contexts}}\DULprodnewline
\DULfirstprodline{|}{\DULsym{(}  s_{{\mathrm{1}}}  \DULsym{,}  s_{{\mathrm{2}}}  \DULsym{)}}{}{}{}{}\DULprodnewline
\DULprodline{|}{\target{q}^\target{T}}{}{}{}{}}

\newcommand{\DULb}{
\DULrulehead{\DULnt{b}  ,\ \pi}{::=}{\DULcom{behaviors}}\DULprodnewline
\DULfirstprodline{|}{ \textsf{Accept} }{}{}{}{}\DULprodnewline
\DULprodline{|}{ \textsf{Reject} }{}{}{}{}}

\newcommand{\DULwstring}{
\DULrulehead{\mathtarget{w}}{::=}{}}

\newcommand{\DULstring}{
\DULrulehead{s}{::=}{}\DULprodnewline
\DULfirstprodline{|}{c_{{\mathrm{1}}} \, .. \, c_{\DULmv{n}}}{}{}{}{}\DULprodnewline
\DULprodline{|}{s_{{\mathrm{1}}}  \doubleplus  s_{{\mathrm{2}}}}{}{}{}{}\DULprodnewline
\DULprodline{|}{\epsilon}{}{}{}{}\DULprodnewline
\DULprodline{|}{\mathtarget{w}}{}{}{}{}}

\newcommand{\DULset}{
\DULrulehead{X}{::=}{}\DULprodnewline
\DULfirstprodline{|}{\DULsym{\{}  \DULnt{top_{{\mathrm{1}}}}  \DULsym{,} \, .. \, \DULsym{,}  \DULnt{top_{\DULmv{n}}}  \DULsym{\}}}{}{}{}{}\DULprodnewline
\DULprodline{|}{\DULsym{\{}  \DULnt{top_{{\mathrm{1}}}}  \DULsym{,} \, .. \, \DULsym{,}  \DULnt{top_{\DULmv{n}}}  \cdots  \DULsym{\}}}{}{}{}{}\DULprodnewline
\DULprodline{|}{ \left\{  \DULnt{top}  \mid  \DULnt{form}  \right\} }{}{}{}{}\DULprodnewline
\DULprodline{|}{ \left\{  \DULnt{judg}  \mid  \DULnt{form}  \right\} }{}{}{}{}\DULprodnewline
\DULprodline{|}{ \left\{  \DULnt{top}  \mid  \DULnt{top'}  \right\} }{}{}{}{}\DULprodnewline
\DULprodline{|}{ \left\{  \DULnt{judg}  \mid  \DULnt{top}  \right\} }{}{}{}{}\DULprodnewline
\DULprodline{|}{ \mathcal{P}( X ) }{}{}{}{}\DULprodnewline
\DULprodline{|}{ \emptyset }{}{}{}{}\DULprodnewline
\DULprodline{|}{X_{{\mathrm{1}}}  \times  X_{{\mathrm{2}}}}{}{}{}{}\DULprodnewline
\DULprodline{|}{X_{{\mathrm{1}}}  \cup  X_{{\mathrm{2}}}}{}{}{}{}\DULprodnewline
\DULprodline{|}{X_{{\mathrm{1}}}  \DULsym{\mbox{$\backslash{}$}}  X_{{\mathrm{2}}}}{}{}{}{}\DULprodnewline
\DULprodline{|}{X_{{\mathrm{1}}}  \rightarrow  X_{{\mathrm{2}}}}{}{}{}{}\DULprodnewline
\DULprodline{|}{ \textsf{Bool} }{}{}{}{}\DULprodnewline
\DULprodline{|}{ \textsf{Nat} }{}{}{}{}\DULprodnewline
\DULprodline{|}{ \textsf{Int} }{}{}{}{}\DULprodnewline
\DULprodline{|}{ \textsf{String} }{}{}{}{}\DULprodnewline
\DULprodline{|}{ \List{ X } }{}{}{}{}\DULprodnewline
\DULprodline{|}{\DULnt{Q}}{}{}{}{}\DULprodnewline
\DULprodline{|}{\Sigma}{}{}{}{}}

\newcommand{\DULtop}{
\DULrulehead{\DULnt{top}}{::=}{}\DULprodnewline
\DULfirstprodline{|}{b}{}{}{}{}\DULprodnewline
\DULprodline{|}{i}{}{}{}{}\DULprodnewline
\DULprodline{|}{X}{}{}{}{}\DULprodnewline
\DULprodline{|}{q}{}{}{}{}}

\newcommand{\DULgrammar}{\DULgrammartabular{
\DULdigit\DULinterrule
\DULnat\DULinterrule
\DULint\DULinterrule
\DULbool\DULinterrule
\DULchar\DULinterrule
\DULform\DULinterrule
\DULPXXS\DULinterrule
\DULPXXT\DULinterrule
\DULsstate\DULinterrule
\DULtstate\DULinterrule
\DULstate\DULinterrule
\DULrepmap\DULinterrule
\DULQ\DULinterrule
\DULAccepting\DULinterrule
\DULFSM\DULinterrule
\DULAlphabet\DULinterrule
\DULTransition\DULinterrule
\DULjudg\DULinterrule
\DULCmp\DULinterrule
\DULS\DULinterrule
\DULT\DULinterrule
\DULCtx\DULinterrule
\DULSCtx\DULinterrule
\DULTCtx\DULinterrule
\DULb\DULinterrule
\DULwstring\DULinterrule
\DULstring\DULinterrule
\DULset\DULinterrule
\DULtop\DULafterlastrule
}}

% defnss
% defns Dullien
%% defn link
\newcommand{\DULdruleDullienXXLink}[1]{\DULdrule[#1]{%
}{
\DULsym{(}   p  \,  r  \,  e   \DULsym{,}   p  \,  o  \,  s  \,  t   \DULsym{)}  \DULsym{[}  s  \DULsym{]}  \DULsym{=}   p  \,  r  \,  e   \doubleplus  s  \doubleplus   p  \,  o  \,  s  \,  t }{%
{\DULdrulename{Dullien\_Link}}{}%
}}

\newcommand{\DULdefnDullienXXlink}[1]{\begin{DULdefnblock}[#1]{$\source{C}^\source{S}  \DULsym{[}  \source{S}  \DULsym{]}  \DULsym{=}  \source{P}$}{}
\DULusedrule{\DULdruleDullienXXLink{}}
\end{DULdefnblock}}

%% defn sequiv

\newcommand{\DULdefnDullienXXsequiv}[1]{\begin{DULdefnblock}[#1]{$q_{{\mathrm{1}}}  \equiv  q_{{\mathrm{2}}}$}{}
\end{DULdefnblock}}

%% defn sstep

\newcommand{\DULdefnDullienXXsstep}[1]{\begin{DULdefnblock}[#1]{$ q  \overstep{ s }  q' $}{}
\end{DULdefnblock}}

%% defn ssteps

\newcommand{\DULdefnDullienXXssteps}[1]{\begin{DULdefnblock}[#1]{$ q  \oversteps{ s }  q' $}{}
\end{DULdefnblock}}


\newcommand{\DULdefnsDullien}{
\DULdefnDullienXXlink{}\DULdefnDullienXXsequiv{}\DULdefnDullienXXsstep{}\DULdefnDullienXXssteps{}}

\newcommand{\DULdefnss}{
\DULdefnsDullien
}

\newcommand{\DULall}{\DULmetavars\\[0pt]
\DULgrammar\\[5.0mm]
\DULdefnss}



==> toyc-text.tex <==
In the appendix we give formal descriptions of the languages referenced in \cref{sec:examples}.

\subsection{$ \IMP $}
\label{app:examples:IMP}

$ \IMP $ syntax:
\begin{align*}
   \intermediate{e} &::= \ottmv{x} ∣  \mathintermediate{ b }   \in   \textsf{Bool}  ∣  \mathintermediate{ n }   \in   \textsf{Nat}  
%        ∣ \alpha \, \intermediate{e} 
          ∣ \intermediate{e} \, \circledast \, \intermediate{e}
        \tag{$ \IMP $ expressions} \\
   \circledast &::= + ∣ × ∣ < ∣ == ∣ ∧ ∣ ∨ \tag{binary operations} \\
%   \alpha &::= ¬ \tag{unary operations} \\
   \intermediate{c} &::= \ottmv{x}  \coloneqq  \intermediate{e} ∣  \OUTPUT{ \intermediate{e} }  ∣  \SKIP  ∣ \intermediate{c}  \ottsym{;}  \intermediate{c}  \\
            &∣  \ifThenElse{ \intermediate{e} }{ \intermediate{c} }{ \intermediate{c} }  ∣  \while{ \intermediate{e} }{ \intermediate{c} } 
            \tag{$ \IMP $ commands}
\end{align*}

\paragraph{Operational semantics}

Given a store $\mathintermediate{\sigma}$, expressions $\intermediate{e}$ evaluate to values $v$; we write this judgment $\mathintermediate{\sigma}  \vdash  \intermediate{e}  \Downarrow  v$. A configuration---a pair of a command and a store $\intermediate{c}  \ottsym{/}  \mathintermediate{\sigma}$---can step to another configuration, possibly outputting a trace of values; this judgment is written $ \intermediate{c}  \ottsym{/}  \mathintermediate{\sigma}  \overstep{ t }  \intermediate{c}'  \ottsym{/}  \mathintermediate{\sigma}' $.
\begin{align*}
    v &::=  \mathintermediate{ b }   \in   \textsf{Bool}  ∣  \mathintermediate{ n }   \in   \textsf{Nat}  \tag{$ \IMP $ values} \\
    \mathintermediate{\sigma} &::= \ottmv{x}  \mapsto  v ∣ \mathintermediate{\sigma}_{{\mathrm{1}}}  \ottsym{,} \, .. \, \ottsym{,}  \mathintermediate{\sigma}_{\ottmv{n}} \tag{$ \IMP $ store} \\
    t &::=  \cdot  ∣ v  \ottsym{,}  t \tag{$ \IMP $ trace}
\end{align*}


\paragraph{Map of $ \IMP $ syntax onto weird machine meta-variables.}

\begin{align*}
    \intermediate{P}^\intermediate{I} &::= \intermediate{c} \tag{$ \IMP $ whole program} \\
    \intermediate{U}^\intermediate{I} &::= \ottsym{(}  \intermediate{c}  \ottsym{,}   \vect{ \ottmv{x_{\ottmv{i}}} }   \ottsym{)} \tag{$ \IMP $ component} \\
    \intermediate{C}^\intermediate{I} &::=  \square^{  \vect{ \ottmv{x_{\ottmv{i}}} }  }  ∣ \intermediate{C}^\intermediate{I}  \ottsym{;}  \intermediate{c} ∣ \intermediate{c}  \ottsym{;}  \intermediate{C}^\intermediate{I} \\
        &∣  \ifThenElse{ \ottnt{e} }{ \intermediate{C}^\intermediate{I} }{ \intermediate{c} }  ∣  \ifThenElse{ \ottnt{e} }{ \intermediate{c} }{ \intermediate{C}^\intermediate{I} }  \\
        &∣  \while{ \ottnt{e} }{ \intermediate{C}^\intermediate{I} } 
        \tag{$ \IMP $ context} \\
\end{align*}





\subsection{$ \ToyC $}
\label{app:examples:toyc}

\paragraph{$ \ToyC $ expressions.}

\begin{align*}
    \source{e} &::= \ottmv{x} ∣  \mathsource{ i } 
%        ∣ \alpha \, \source{e}
        ∣ \source{e}_{{\mathrm{1}}} \, \circledast \, \source{e}_{{\mathrm{2}}}
        ∣ \ottkw{NULL} ∣ \ottsym{*}  \source{e} ∣ \ottsym{\&}  ℓ^{v} \tag{$ \ToyC $ expressions} \\
    ℓ^{v} &::= \ottmv{x} ∣ \ottsym{*}  ℓ^{v} \tag{$ \ToyC $ l-values}
\end{align*}
L-values $ℓ^{v}$ are either variables or pointers. Expressions can be assigned types $\mathsource{\tau}$, which are either simple types (integers and pointers) or arrays of simple types. The typing rules for expressions are given in \cref{fig:ToyExpressions}.
\begin{align*}
  \mathsource{\tau}  &::= \mathsource{\sigma} ∣ \mathsource{\sigma}  \ottsym{[}  n  \ottsym{]} \tag{$ \ToyC $ types}\\
  \mathsource{\sigma} &::=  \textsf{Int}  ∣ \ottsym{*}  \mathsource{\tau} \tag{$ \ToyC $ simple types}
\end{align*}

\begin{figure*}
\[ \begin{array}{c}
    \CdruleToyCXXtypeXXvar{}
  \qquad
    \CdruleToyCXXtypeXXInt{}
  \\ \\
    \CdruleToyCXXtypeXXNULL{}
  \qquad
    \CdruleToyCXXtypeXXBinop{}
  \\ \\
    \CdruleToyCXXtypeXXDereference{}
  \qquad
    \CdruleToyCXXtypeXXAddress{}
\end{array} \]
\caption{Typing rules for expressions in $ \ToyC $, excluding unary and binary operations.}
\label{fig:ToyExpressions}
\end{figure*}


\paragraph{$ \ToyC $ syntax.}

Procedure declarations $\source{pd}$ map procedure identifiers $p$ to commands $\source{c}$ while specifying the types of their arguments as well as any local variables used in the procedure. Note that arguments to procedures must all have simple types. A global store is a list of procedure declarations, such that no two names overlap, and one procedure is called $ \texttt{main} $.
\begin{align*}
    \source{c} &::= p  \ottsym{(}  \source{e}_{{\mathrm{1}}}  \ottsym{,} \, .. \, \ottsym{,}  \source{e}_{\ottmv{n}}  \ottsym{)} ∣  ℓ^{v}  ≔  \source{e}  ∣  \OUTPUT{ \source{e} } 
                ∣  \SKIP  ∣ \source{c}  \ottsym{;}  \source{c} \\
                &∣  \ifThenElse{ \source{e} }{ \source{c} }{ \source{c} }  ∣  \while{ \source{e} }{ \source{c} } 
                \tag{$ \ToyC $ commands} \\
    \source{pd} &::= p  \ottsym{(}   \vect{ \ottmv{x_{\ottmv{i}}}  \ottsym{:}  \mathsource{\sigma}_{\ottmv{i}} }   \ottsym{;}   \vect{ \ottmv{y_{\ottmv{j}}}  \ottsym{:}  \mathsource{\tau}_{\ottmv{j}} }   \ottsym{)}  \ottsym{\{}  \source{c}  \ottsym{\}}
                \tag{$ \ToyC $ procedure declarations} \\
    p &∈  \textsf{String}  \tag{Procedure identifiers} \\
    \mathsource{G} &::= \ottsym{\{}  \source{pd}_{{\mathrm{1}}}  \ottsym{,} \, .. \, \ottsym{,}  \source{pd}_{\ottmv{n}}  \ottsym{\}} 
                \tag{$ \ToyC $ global store}
\end{align*}


\begin{theorem}
  The compiler from $ \IMP $ to $ \ToyC $ is modular. It is correct for whole programs.
\end{theorem}
\begin{proof}

   The compiler is correct for whole programs if, for all whole $ \IMP $ programs $\intermediate{P}^\intermediate{I}$, it is the case that $ \brelates{  \ibehav{ \intermediate{P}^\intermediate{I} }  }{  \tbehav{  \compile[  \intermediate{P}^\intermediate{I}  ]  }  } $. This can be observed by induction on commands $\intermediate{c}$.
\end{proof}



%% \subsection{Examples}

%% Let $\mathsource{G}$ be the ToyC program composed of the following two components:
%% \begin{lstlisting}[language=C]
%% main(int o, int ret) { vulnerable(o,&ret); }
%% vulnerable(int o, *int ret) {
%%   int v;
%%   int[1] p;

%%   v = 0;
%%   p = p+o;
%%   *p = 1;
%%   &ret = v;
%%   output(*ret);
%% }
%% \end{lstlisting}
%% Then $ \texttt{main}  ∈  \textsf{Exploit} (\texttt{vulnerable})$. 

%% If the input $o$ is $0$, then this program will output $0$ in $\ToyC$; if $o$ is anything other than $0$, it will get stuck.
%% \[
%%      \sbehav{ \mathsource{G} }  = \ottsym{\{}  \ottsym{\{}  \ottsym{0}  \ottsym{\}}  \ottsym{\}}.
%% \]
%% In fact, we can define a property of behaviors that holds for any non-trivial context $\source{C}^\source{S}$ when linked with $\texttt{vulnerable}$:
%% \[
%%     \mathsource{ \mathbb{B} }_{{\mathrm{0}}} ≜ \{ \target{t}^\target{T} ∣ 0 ∈ \target{t}^\target{T} \}.
%% \]
%% \begin{lemma}
%%     For all non-trivial $\ToyC$ contexts $\source{C}^\source{S}$, $\behav*{\source{C}^\source{S}[\texttt{vulnerable}]} ∈ \mathsource{ \mathbb{B} }_{{\mathrm{0}}}$.
%% \end{lemma}
%% \begin{proof}
%%     If $\source{C}^\source{S}$ is non-trivial, then it invokes $\texttt{vulnerable}$ on some input, which outputs $0$. (Recall that the behavior is only defined if the program terminates in an ending state.) Thus, if $\source{C}^\source{S}[\texttt{vulnerable}]$ outputs $\target{t}^\target{T}$, $0$ must always occur somewhere in $\target{t}^\target{T}$.
%% \end{proof}

%% However, the behavior of $⟦\mathsource{G}⟧$ is quite different. In particular, if the value of $o$ passed in is 4, then the call to $\texttt{vulnerable}$ will redirect $p$ to the address of $v$, the statement $*p[0] = 1$ is equivalent to $v=1$, and so the program will output 1.
%% \[
%%      \behav{\ottsym{⟦}  \mathsource{G}  \ottsym{⟧(}  \target{PC}  \ottsym{,}  \target{SP}  \ottsym{)(}  \ottsym{4}  \ottsym{,}  \ottsym{0}  \ottsym{)}} = \ottsym{\{}  \ottsym{\{}  \ottsym{1}  \ottsym{\}}  \ottsym{\}}.
%% \]

%% Note that $\mathsource{ \mathbb{B} }_{{\mathrm{0}}}$ is a trace property, so $ \texttt{main}  ∈  \textsf{T}  \textsf{Exploit}  $.


%% \jpnote{Come up with some examples based on a limited attacker model, which is not relevant above.}

\subsection{$ \ToyH $}

As described in \cref{sec:examples}, $ \ToyH $ is a \emph{toy hardware} language on which toy assembly code can be executed and observed by a user. As such, $ \ToyH $ is a meta-language in the style of $ \IMP $ that is able to execute arbitrary $ \ToyA $ configurations and get back as input both the output from the execution as well as the number of steps that configuration took.
\begin{align*}
    \hardware{e} &::= \ottmv{x} ∣  \hardware{ b }   \in   \textsf{Bool}  ∣  \hardware{ i }   \in   \textsf{Int} 
                 %∣ \alpha \, \hardware{e} 
                  ∣ \hardware{e}_{{\mathrm{1}}} \, \circledast \, \hardware{e}_{{\mathrm{2}}}
                 \tag{$ \ToyH $ expressions}
                 \\
    %% \alpha &::= ⋯ ∣  \pi_1  ∣  \pi_2  
    %%             \tag{unary operators} \\
    \hardware{c} &::= \ottmv{x}  \coloneqq  \hardware{e}  ∣  ( \ottmv{x_{{\mathrm{1}}}} , \ottmv{x_{{\mathrm{2}}}} ) ≔ \texttt{get\_info}( \target{P}^\target{T} ) 
                ∣  \OUTPUT{ \hardware{e} }  ∣  \SKIP  ∣ \hardware{c}_{{\mathrm{1}}}  \ottsym{;}  \hardware{c}_{{\mathrm{2}}} \\
               &∣  \ifThenElse{ \hardware{e} }{ \hardware{c}_{{\mathrm{1}}} }{ \hardware{c}_{{\mathrm{0}}} }  
                ∣  \while{ \hardware{e} }{ \hardware{c} }  
                \tag{$ \ToyH $ commands}
\end{align*}

A component in $ \ToyH $ is just a component in $ \ToyA $, and an attacking context is a $ \ToyH $ program with a hole for such $ \ToyA $ components. All holes in the context will be filled in with the same $ \ToyH $ component.
\begin{align*}
    \hardware{P}^\hardware{H} &::= \hardware{c} \tag{$ \ToyH $ whole program} \\
    \hardware{U}^\hardware{H} &::= \target{U}^\target{T} \tag{$ \ToyH $ components} \\
    \hardware{A}^\hardware{H} &::=  ( \ottmv{x_{{\mathrm{1}}}} , \ottmv{x_{{\mathrm{2}}}} ) ≔ \texttt{get\_info}( \target{C}^\target{T} [\square]) 
            ∣ \hardware{A}^\hardware{H}  \ottsym{;}  \hardware{c} ∣ \hardware{c}  \ottsym{;}  \hardware{A}^\hardware{H}
            ∣  \ifThenElse{ \hardware{e} }{ \hardware{A}^\hardware{H} }{ \hardware{c} } 
            ∣  \ifThenElse{ \hardware{e} }{ \hardware{c} }{ \hardware{A}^\hardware{H} } 
            ∣  \while{ \hardware{e} }{ \hardware{A}^\hardware{H} } 
            \tag{$ \ToyH $ attacks}
\end{align*}

\subsection{Compiler from $ \ToyA $ to $ \ToyH $}

The compiler simply injects $ \ToyA $ programs to $ \ToyH $:
\begin{align*}
     \compile[  \target{P}^\target{T}  ]^{x,y}  &≜  ( \ottmv{x_{{\mathrm{1}}}} , \ottmv{x_{{\mathrm{2}}}} ) ≔ \texttt{get\_info}( \target{P}^\target{T} ) 
\end{align*}



